NAGphormer: A Tokenized Graph Transformer for Node Classification in Large Graphs

The graph Transformer emerges as a new architecture and has shown superior performance on various graph mining tasks. In this work, we observe that existing graph Transformers treat nodes as independent tokens and construct a single long sequence composed of all node tokens so as to train the Transformer model, causing it hard to scale to large graphs due to the quadratic complexity on the number of nodes for the self-attention computation. To this end, we propose a Neighborhood Aggregation Graph Transformer (NAGphormer) that treats each node as a sequence containing a series of tokens constructed by our proposed Hop2Token module. For each node, Hop2Token aggregates the neighborhood features from different hops into different representations and thereby produces a sequence of token vectors as one input. In this way, NAGphormer could be trained in a mini-batch manner and thus could scale to large graphs. Moreover, we mathematically show that as compared to a category of advanced Graph Neural Networks (GNNs), the decoupled Graph Convolutional Network, NAGphormer could learn more informative node representations from the multi-hop neighborhoods. Extensive experiments on benchmark datasets from small to large are conducted to demonstrate that NAGphormer consistently outperforms existing graph Transformers and mainstream GNNs. Code is available at https://github.com/JHL-HUST/NAGphormer.

==> 5RW.tex <==


\subsection{Graph Transformers}\label{rw:gfs}
There are several efforts 
to generalize transformer neural networks~\citep{Transformer} to graph-structured data. Similar to the positional encoding in the original Transformer, some notable works compress the graph structure into positional encoding to capture the topological information. 
Dwivedi~\etal~\citep{GT} utilize Laplacian eigenvectors to represent positional encodings and fuse them with the raw attribute of nodes as the input of Transformer.
Derived from~\citep{GT}, Devin~\etal~\citep{SAN} leverage the full spectrum of Laplacian matrix to learn the positional encodings.
In addition to representing structural information by the eigenvectors, Ying~\etal~\citep{Graphormer} propose a spatial encoding method that model the structural similarity of node pairs based on their shortest path lengths. Wu~\etal~\citep{GraphTrans} regard GNNs as an auxiliary module to extract local structural information of nodes and further feed them into the Transformer to learn long-range pairwise relationships. 
Besides, by modeling edge features in chemical and molecular graphs, Dwivedi~\etal~\citep{GT} extend graph Transformers to edge feature representation by injecting them into the self-attention module of Transformer.

Nevertheless, like the original Transformer, these aforementioned methods adopt the fully-connected attention mechanism upon all node pairs, in which the spatial complexity is quadratic with the number of nodes. 
Such high cost makes these methods hard to handle graph mining task on large-scale networks with millions of nodes. 
Recent work~\citep{gophormer} samples several ego-graphs of each node and then utilize Transformer to learn node representations on these ego-graphs for reducing the computational cost of the model training.
However, the sampling process is also time-consuming in large graphs.
Moreover, the sampled ego-graphs only contain limited neighborhood information due to the fixed and small graph size for all nodes, which is insufficient to learn the informative node representations.

%scalable GNNs
\subsection{Scalable Graph Neural Networks}\label{SGNN}
Graph Neural Networks (GNNs) have become a powerful technique to model graph-structured data. % in recent years. 
Based on the message passing framework, typical GNNs~\citep{GCNII,SimpGNN,GCN,GAT} require the entire adjacency matrix as the input during training. In this way, when applying to large-scale graphs, the cost of training is too high to afford. 
To generalize GNNs to large-scale networks and meanwhile reduce the training cost, 
a common approach is to design a sampling strategy. Existing strategies can be divided into two categories: node sampling-based methods~\citep{GraphSAGE, FastGCN, LADIES} that aim at reducing the number of neighborhood nodes, and graph sampling-based methods~\citep{ClusterGCN, GraphSAINT} that dedicate to decrease the input graph size. 
Besides the sampling strategy, recent studies have developed a variety of approximate propagation methods to accelerate the message passing process, such as Approximate Personalized PageRank~\citep{PPRGo}, Localized Bidirectional Propagation~\citep{GBP} and Generalized Forward Push~\citep{Grand+}. 
However, by designing various sampling-based or approximation-based methods to reduce the training cost, these models will inevitably lead to information loss, and somehow restrict their performance on large-scale networks. 







